PKDGRAV3: Beyond Trillion Particle Cosmological Simulations for the Next Era of Galaxy Surveys

We report on the successful completion of a 2 trillion particle cosmological simulation to z=0 run on the Piz Daint supercomputer (CSCS, Switzerland), using 4000+ GPU nodes for a little less than 80h of wall-clock time or 350,000 node hours. Using multiple benchmarks and performance measurements on the US Oak Ridge National Laboratory Titan supercomputer, we demonstrate that our code PKDGRAV3, delivers, to our knowledge, the fastest time-to-solution for large-scale cosmological N-body simulations. This was made possible by using the Fast Multipole Method in conjunction with individual and adaptive particle time steps, both deployed efficiently (and for the first time) on supercomputers with GPU-accelerated nodes. The very low memory footprint of PKDGRAV3 allowed us to run the first ever benchmark with 8 trillion particles on Titan, and to achieve perfect scaling up to 18000 nodes and a peak performance of 10 Pflops.

==> justification.tex <==
\section{Justification}
% 50 words maximum
% indicate what implementation or performance “high watermark” was achieved (rather than the science that was enabled)
With PKDGRAV3 it is possible to run cosmological $N$-body simulations at
unprecedented resolution -- as high as 8~trillion particles on Titan --
and such a simulation will take less than three days which is an
order of magnitude decrease in the time-to-solution compared
with other existing codes.

